Recovery Guarantees for Quadratic Tensors with Sparse Observations

We consider the tensor completion problem of predicting the missing entries of a tensor. The commonly used CP model has a triple product form, but an alternate family of quadratic models, which are the sum of pairwise products instead of a triple product, have emerged from applications such as recommendation systems. Non-convex methods are the method of choice for learning quadratic models, and this work examines their sample complexity and error guarantee. Our main result is that with the number of samples being only linear in the dimension, all local minima of the mean squared error objective are global minima and recover the original tensor. We substantiate our theoretical results with experiments on synthetic and real-world data, showing that quadratic models have better performance than CP models where there are a limited amount of observations available.

==> logistic.tex <==
\section{The TransE Model}

Our techniques can also be used to obtain sample complexity bounds for other quadratic tensor models.
In this section we demonstrate an example, called the TransE model, which is commonly used for modeling multi-relational data.

We now describe the idea behind the TransE model.
Let $I$ denote the set of all entities and $R$ denote the set of relationships
Let $n = \abs{I} + \abs{R}$.
Consider a triple $(i, l, j) \in I \times R \times I$, where $i$ and $j$ correspond to two entities, and $l$ corresponds to a relationship.
An example is (Rome, is capital of, Italy).
The idea of the TransE model is to learn an embedding $u$ for every entity and relationship.
Intuitively, $i$ and $j$ are related by $l$ if $\norm{u_i + u_l - u_j}$ is small,
where $u_i, u_l, u_j$ are the embedding vectors of $i, l, j$.

\begin{assumption}
	Denote by $U^{\star} \in \real^{n \times d}$ as the embedding matrix of all the entities and relationships.
	We will assume that $\tr(U^{\star}{U^{\star}}^{\top}) \le O(r)$.
\end{assumption}

The assumption says that the spectrum of embedding matrix $UU^{\top}$ consists of at most $O(r)$ singular values which are large (say at least $0.1$), while all the other singular values are small.

Let $T^{\star}$ denote a 3rd order tensor with dimension $\abs{I} \times \abs{R} \times \abs{I}$.
Given the embedding matrix $U^{\star}$, the $(i, l, j)$-th entry of $T^{\star}$ is equal to $\norm{U_i + U_l - U_j}^2$.
Suppose that we are given a set of $\Omega$ labeled triples, our next assumption describes way in which the triples are generated from $T^{\star}$.

\begin{assumption}
	For each triple $(i, l, j) \in I \times R \times I$,
	we observe that
	\[ \Pr(y_{i, l, j}) = \begin{cases}
		0 & \text{with probability}~f(T_{i, l, j}),\\
		1 & \text{with probability}~1 - f(T_{i, l, j}).
		\end{cases}
	\]
\end{assumption}

As an example, consider $f(x) = \frac{e^x} {1 + e^x}.$



==> pairwise_1norm.tex <==
\section{Recovery Guarantee for Quadratic Tensor Models}
\label{sec_main}

In this section, we consider the recovery of quadratic tensor models given only partial observations.
Recall that we observe $m$ uniformly random entries from the unknown tensor $T$.
Let $\Omega \in [d]^3$ denote the indices of the set of observed entries.
Given the set of observations $\Omega$, our goal is to recover $T$.
We first review the definition of local optimality conditions.

\begin{definition}
	(Local minimum) Suppose that $U$ is a local minimum of $f(U)$, then we have that
	$\nabla f(U) = \zeroMatrix$ and $\nabla^2 f(U) \gematrix \zeroMatrix$.
\end{definition}

We focus on the following non-convex formulation
over the set of $X,Y,Z \subseteq \real^{d \times R}$.
\begin{align}
	\min_{X,Y,Z \subseteq \real^{d \times R}} h(X,Y,Z) = & \frac 1 m \sum_{(i, j, k) \in \Omega} \bigbrace{\sum_{l=1}^R \kappa(X_{i,l}, Y_{j,l}, Z_{k,l}) - T_{i, j, k}}^2 \\
	+ & \lambda (\normFro{X}^{2} + \normFro{Y}^2 + \normFro{Z}^2) \\
	+ & \inner{[X;Y;Z]}{C \dot [X;Y;Z]},
\end{align}
where $\lambda$ is a fixed value which will be determined later,
and $C \in \cS_{3d}^+$ is a random PSD matrix with spectral norm at most $\lambda$.
Here the $l_2$ regularier is to ensure good generalization performance.
And the random matrix $C$ acts as a small perturbation to the objective.
Our main result is described below.

\begin{theorem}\label{thm_main}
	Let $T^{\star} \subseteq \real^{d \times d \times d}$ be a quadratic tensor defined by factors $A^{\star}, B^{\star}, C^{\star} \subseteq \real^{d \times r}$ and a quadratic function $\kappa$ with kernel $K \subseteq \real^{3 \times 3}$.
	Assume that $\normFro{A^{\star}} + \normFro{B^{\star}} + \normFro{C^{\star}} \le \alpha$.
	We are given a uniformly random subset of $m$ entries $\Omega \subseteq [d]^3$ from $T^{\star}$, along with their values.
	Let $C \in \cS_{3d}^+$ be a random PSD matrix with spectral norm at most $\lambda = $.
	Let $m \gtrsim d (\log d) / \varepsilon^2$ and $R \ge \sqrt{2m + 2d}$.

	For any local minimum $X,Y,Z$ of $f$, with high probability over the randomness of $\Omega$ and $C$, by reconstructing $\hat{T}_{i, j, k} = \sum_{l=1}^R \kappa(X_{i,l}, Y_{j,l}, Z_{k,l})$, we have:
	\[ \frac 1 {d^3} \sum_{1\le i,j,k \le d} \abs{\hat{T}_{i,j,k} - T^{\star}_{i,j,k}} \lesssim \alpha \varepsilon. \]
\end{theorem}

Note that the low rank case of Theorem \ref{thm_intro} is a corollary of Theorem \ref{thm_main}.
This is because when the rank of $A$ is $r$ and $\norm{e_i^{\top} A} \le \sqrt{\mu r / d}$ for all $i$, we have that $\normFro{A} \le \sqrt{\mu r}$.
The same holds for $B$ and $C$.
Hence Theorem \ref{thm_intro} follows by setting $\alpha = \sqrt{\mu r}$ in Theorem \ref{thm_main}.

As another example, suppose that $A^{\star}, B^{\star}, C^{\star}$ are all sampled independently from $\cN(0, 1 / \sqrt d)$.
In this case, it is easy to verify that $\alpha = O(r (\log d) / d)$.
When $m \gtrsim d r^4 \log^3 d$, we have that the average MSE of $\hat{T}$ is at most $O(\varepsilon/ d^2)$.
Note that every entry of $T^{\star}$ is on the order of $1/d$ based on the quadratic model.
Hence $\hat{T}$ can recover $T^{\star}$ for most entries up to a relative MSE of $\varepsilon$.

The first technical complication of analyzing $h(X,Y,Z)$ is that the three factors are asymmetric.
Therefore to simplify the analysis, we first reduce the problem to a symmetric problem, by viewing the search space as $[X; Y; Z]$ instead.
We then show that all local minima of $g(X,Y,Z)$ are global minima, via an interesting connection between SDPs and ther low-rank Burer-Monteiro formulation \cite{BVB16}.
We use smoothed analysis to \todo{phrasing}.
This will ensure that any local minima incurs a small MSE on $\Omega$.
Then we bound the generalization error through the regularization added to $g(X,Y,Z)$.

\paragraph{Local optimality} Before proceeding, we introduce several notations needed in the proof.
Denote by $U^{\star} = [A^{\star}; B^{\star}; C^{\star}] \subseteq \real^{3d \times r}$ as the three factors stacked vertically.
Let $X^{\star} = U^{\star} {U^{\star}}^{\top}$.
For each triple $t = (i, j, k) \in [d]^3$, denote by $A_t \subseteq \real^{3d \times 3d}$ as a sensing matrix such that $\inner{A_t}{X^{\star}} = T^{\star}_{i, j, k}$.
Specifically, we have that $A_t$ restricted to the row and column indices $i, j+d, k+2d$ is equal to $K$ (the kernel matrix of $\kappa$), and $0$ otherwise.
\todo{draw pic?}
We can rewrite $g(X, Y, Z)$ as follows:
\begin{align}
	f(U) = \frac 1 m \sum_{t \in \Omega} \inner{A_t}{UU^{\top} - X^{\star}}^2 + \lambda_1 \normFro{U}^2
	+ \lambda_2 \sum_{i=1}^{3d} q_{\alpha}(\norm{e_i^{\top} U})
	+ \inner{C}{UU^{\top}},
\end{align}
where $U = [X;Y;Z] \subseteq \real^{3d \times R}$.

We will use the following Proposition during the proof.
\begin{proposition}[Proposition 4 in Bach et al. \cite{BMP08}]\label{prop_deficient}
		Let $g$ be a twice differentiable function convex function over $\cS_d^+$.
		If the function $h: U \rightarrow g(UU^{\top})$ defined over $U \subseteq d \times d'$ has a local minimum at a rank deficient matrix $V$, then $VV^{\top}$ is a global minimum of $g$.
\end{proposition}

Here we show that there is no bad local minima in the landscape of $g(U)$.
\begin{lemma}\label{lem_local}
	In the setting of Theorem \ref{thm_main}, we have that any local minimum $V$ of $g(U)$ is a global minimum with high probability.
\end{lemma}

\begin{proof}
	Since $V$ is a local minimum of $f(U) + \inner{C}{UU^{\top}}$, we have that $\nabla g(U) = \zeroMatrix$.
	We will show that $\rank(V) < k$, hence by Proposition \ref{prop_deficient}, $V$ is a global minimum of $g(U)$.
	Assume that $\rank(V) = k$.
	By $\nabla g(U) = \zeroMatrix$, we obtain:
	\begin{align}
		& \left(\sum_{t \in \Omega} z_t A_t
		+ \sum_{i = 1}^d w_i e_i e_i^{\top}
		+ \lambda_1 \id + C \right) U = \zeroMatrix, \\
		&\quad\quad \text{where}~ w_i = \frac{4\lambda_2 (\norm{e_i^{\top} U} -\alpha)^3} {\norm{e_i^{\top} U}} \ind{\norm{e_i^{\top} U} \ge \alpha}, \\
		&\quad\quad \text{and}~ z_t = \frac 2 m \inner{A_t}{UU^{\top} - X^{\star}}
	\end{align}
	Denote by
	\begin{align}
		& M(w, z) = \sum_{i=1}^d w_i e_i e_i^{\top} + \sum_{t \in \Omega} z_t A_t, \text{and} \\
		& \cA = \bigset{X - M(w, z) - \lambda_1 \id : X \in \cS_{3d}, XU = \zeroMatrix, w \in \real^d, z \in \real^m}.
	\end{align}
	The set $\cA$ is a manifold and we have that $C \in \cA$.
	Note that $X$ is a symmetric matrix in the null space of $U$,
	recalling that $A_t$ is a symmetric matrix, for any $t \in [d]^3$.
	Since the rank of the null space is $n - k$, the dimension of such $X$ is $\frac{3d(3d+1)} 2 - \frac{k(k+1)} 2$.
	Together with $w$ and $z$, we have that the dimension of $\cA$ is
	\[ \frac{3d(3d+1)} 2 - \frac{k(k+1)} 2 + m + d. \]
	We have assumed that $k \ge \sqrt{2m + 2d}$, implying that the dimension of $\cA$ is less than $\frac{3d(3d+1)} 2$.
	However, the probability that a random PSD matrix $C$ falls in such a set $\cA$ only happens with probability zero.
	Hence with high probability, the rank of $V$ is less than $k$.
\end{proof}

\paragraph{Rademacher complexity}
Next we bound the Rademacher complexity of quadratic tensor models.
We first introduce some notations.
For any $S \subseteq [d]^3$, denote by
\[ \cL_{S}(X) = \frac 1 {\abs{S}} \sum_{t \in S} \abs{\inner{A_t}{X - X^{\star}}}. \]
And let $\cG$ denote the set of matrices as follows.
\begin{align*}
	\cG \define \bigset{X \in \cS_{3d}^+ : \tr(X) \le \alpha}.
\end{align*}
We bound the Rademacher complexity of $\cG$ in the following Lemma.
\begin{lemma}\label{lem_rade}
	In the setting of Theorem \ref{thm_main}, we have that with high probability over the randomness of $\Omega$,
	\[ \sup_{X \in \cG} \abs{\cL_{\Omega}(X) - \cL_{[d]^3}(X)} \le c \norm{K}_1 \alpha \varepsilon, \]
	where $c$ is a certain fixed constant.
\end{lemma}

\begin{proof}%
	We will prove the following inequality:
	\begin{align}\label{eq_markov}
		\exarg{\Omega}{\sup_{X \in \cG} \abs{\cL_{\Omega}(X) - \cL_{[d]^3}(X)}}
	\le {c \norm{K}_1 \alpha \sqrt{\frac d m + \frac{d^{2}\log d}{m^2}}}
		\le \frac {c \norm{K}_1 \alpha \varepsilon} {\sqrt{\log d}},
	\end{align}
	since $m \ge d \log d / \varepsilon^2$.
	Based on the above inequality, we can obtain that by Markov's inequality, the probability that $\sup_{X \in \cG} \abs{\cL_{\Omega}(X) - \cL_{[d]^3}(X)} > c \norm{K}_1 \alpha \varepsilon$ happens with probability $1 / \sqrt{\log d}$.
	In the following we will prove Equation \eqref{eq_markov}.
	Let $\Omega'$ denote a set of $m$ independent samples from $[d]^3$.
	Clearly,
	\[ \exarg{\Omega}{\cL_{\Omega}(X)} = \exarg{\Omega'}{\cL_{\Omega'}(X)}. \]
	By concavity, we have:
	\begin{align}
		& \exarg{\Omega}{\sup_{X \in \cG} \abs{\frac 1 m \sum_{t \in \Omega} \abs{\inner{A_t}{X - X^{\star}}}  - \exarg{\Omega'}{\frac 1 m \sum_{t' \in \Omega'} \abs{\inner{A_{t'}}{X - X^{\star}}}} }} \nonumber \\
		\le & \exarg{\Omega, \Omega'}{\sup_{X \in \cG} \abs{\frac 1 m \sum_{t \in \Omega} \abs{\inner{A_t}{X - X^{\star}}} - \frac 1 m \sum_{t' \in \Omega'} \abs{\inner{A_{t'}}{X - X^{\star}}}}}
		\label{eq_jensen}
	\end{align}
	Let $\set{\sigma_i}_{i=1}^m$ denote $m$ i.i.d. Rademacher random variables.
	By the symmetry of $\Omega$ and $\Omega'$, Equation \eqref{eq_jensen} is equal to:
	\begin{align}
		& \exarg{\Omega, \Omega', \sigma}{\sup_{X \in \cG} \abs{\frac 1 m \sum_{l=1}^m \sigma_l \times \bigbrace{\abs{\inner{A_{t_l}}{X - X^{\star}}} - \abs{\inner{A_{t'_l}}{X - X^{\star}}}} }} \nonumber \\
		& \le	2 \times \exarg{\Omega, \sigma}{\sup_{X \in \cG} \abs{\frac 1 m \sum_{l=1}^m \sigma_l \abs{\inner{A_{t_l}}{X - X^{\star}}}}} \nonumber \\
		& = 2 \times \exarg{\Omega, \sigma}{\sup_{X \in \cG} \abs{\frac 1 m \sum_{l=1}^m \sigma_l \inner{A_{t_l}}{X - X^{\star}}}} \nonumber \\
		& = \frac 2 m \times \exarg{\Omega, \sigma}{\sup_{X \in \cG}\inner{\sum_{l=1}^m \sigma_{t_l} A_{t_l}}{X - X^{\star}}}, \label{eq_spec}
	\end{align}
	where the second inequality uses triangle inequality and the symmetry between $\Omega$ and $\Omega'$.
	Denote by $E = \sum_{l=1}^m \sigma_{t_l} A_{t_l}$.
	We have that
	\[ \inner{E}{X - X^{\star}} \le \norm{E} \times \normNuclear{X - X^{\star}}. \]
	And \[ \normNuclear{X - X^{\star}} \le \normNuclear{X} + \normNuclear{X^{\star}} = \tr(X + X^{\star}), \]
	because both $X$ and $X^{\star}$ are PSD.
	When $X \in \cG$, we know that $\tr(X) \le \alpha$.
	By assumption, we also have that $\tr(X^{\star}) \le \alpha$.
	Hence Equation \eqref{eq_spec} can be bounded by,
	\begin{align}\label{eq_res}
		\frac {4\alpha} {m} \times \exarg{\Omega, \sigma}{\bignorm{\sum_{l=1}^m \sigma_{t_l} A_{t_l}}}.
	\end{align}
	To handle the above expecation, we will use the following fact, which is proved in the proof of Lemma 1 in \cite{DPVW14}.

	\begin{fact}\label{fact}
		Let $\Omega = \set{(i_1, j_1), (i_2, j_2), \dots, (i_m, j_m)}$ be a set of $m$ uniformly random samples from a $d$ by $d$ matrix.
		Let $Z_{k}$ be the indicator matrix for $(i_k, j_k)$, in other words, the $(i_k, j_k)$-th entry of $Z$ is 1, and 0 otherwise.
		Let $\sigma_{k}$ denote Rademacher random variables, for $1 \le k \le m$.
		We have that $\exarg{\Omega,\sigma}{\norm{\sum_{k=1}^m \sigma_k Z_k}} \le O(\sqrt{d m + d^2 \log d})$.
	\end{fact}

	To see how to use the above fact in our setting,
	observe that $A_t$ contrains 9 nonzero indicator entries, for every $t \in [d]^3$.
	If we divide $A_t$ into the 9 $d$ by $d$ submatrices, then there is exactly 1 indicator entry in each submatrix.
	Hence we can use Fact \ref{fact} to bound the contribution of each $d$ by $d$ submatrix.
	\footnote{For diagonal blocks, we cannot use Fact \ref{fact} exactly. However, the result follows from the proof in Lemma 1 in \cite{DPVW14} as well.}
	To sum up, we conclude that
	\[ \exarg{\Omega,\sigma}{\norm{\sum_{l=1}^m \sigma_{t_l} A_{t_l}}} \le O(\norm{K}_1 \sqrt{d m + {d^2 \log d}}). \]
	By combining Equation \eqref{eq_spec} and \eqref{eq_res}, the proof is complete.
\end{proof}

Lastly, we finish the proof of Theorem \ref{thm_main}.

\begin{proof}[Proof of Theorem \ref{thm_main}]
	By Lemma \ref{lem_local}, we have that $V$ is a global minimum of $g(U)$.
	In particular, this implies that
	\[ g(V) \le g(U^{\star}) \le (\lambda_1 + \norm{C}) \normFro{U^{\star}}^2 \le 2\lambda_1 \normFro{U^{\star}}, \]
	since $\normFro{C} \le \lambda_1$.
	In particular, this implies that the training error $\cL_{\Omega}(VV^{\top}) \le 2\lambda \normFro{U^{\star}}^2 \lesssim \norm{K}_1 \alpha^2 \varepsilon$ by the setting of $\lambda_1$.

	We also obtain that $\norm{e_i^{\top} V} \le \sqrt 2 \alpha$ by the setting of $\lambda_2$.
	Hence we conclude that the $(i,i)$-th entry of $VV^{\top}$ is at most $2\alpha$ and its trace is at most $2d\alpha$.
	This implies that $VV^{\top} \in \cG$.
	Hence by Lemma \ref{lem_rade}, the generalization error is also bounded by $\bigo{\norm{K}_1 \alpha^2 \varepsilon}$.
	The proof is complete.
\end{proof}


\paragraph{Discussion.} Room for improvement over k?








==> pairwise_copy.tex <==
\section{Recovery Guarantee for Quadratic Tensor Models}
\label{sec_main}

In this section, we consider the recovery of quadratic tensor models given only partial observations.
Recall that we observe $m$ uniformly random entries from the unknown tensor $T$.
Let $\Omega \in [d]^3$ denote the indices of the set of observed entries.
Given the set of observations $\Omega$, our goal is to recover $T$.
We first review the definition of local optimality conditions.

\begin{definition}
	(Local minimum) Suppose that $U$ is a local minimum of $f(U)$, then we have that
	$\nabla f(U) = \zeroMatrix$ and $\nabla^2 f(U) \gematrix \zeroMatrix$.
\end{definition}

We focus on the following non-convex formulation
over the set of $X,Y,Z \subseteq \real^{d \times R}$.
\begin{align}
	\min_{X,Y,Z \subseteq \real^{d \times R}} h(X,Y,Z) = & \frac 1 m \sum_{(i, j, k) \in \Omega} \bigbrace{\sum_{l=1}^R \kappa(X_{i,l}, Y_{j,l}, Z_{k,l}) - T_{i, j, k}}^2 \\
	+ & \lambda_1 (\normFro{X}^{2} + \normFro{Y}^2 + \normFro{Z}^2) \\
	+ & \lambda_2 \sum_{i=1}^d q_{\alpha}(\norm{e_i^{\top} U}),
\end{align}
where $q_{\alpha}(x) = (\abs{x} - \sqrt{\alpha})^4 \ind{x \ge \sqrt{\alpha}}$,
$\lambda_1 = \bigo{\frac{\norm{K} \mu} {d^2} \sqrt{\frac d m}}$ and $\lambda_2 = \frac{d^2 r} {\mu^4} \lambda_1$ (the reason for the setting will be clear later).
Here $q_{\alpha}(x)$ acts as a regularizer which penalizes the rows of $A,B,C$ whose norms are larger than $\sqrt{\alpha}$.
And the $l_2$ regularier is to ensure good generalization performance.
It is not hard to verify that $q_{\alpha}(x)$ is twice differentiable.
And it follows that $f$ is a twice differentiable function.
Our main result is described below.

\begin{theorem}\label{thm_main}
	Let $T^{\star} \subseteq \real^{d \times d \times d}$ be a quadratic tensor defined by factors $A^{\star}, B^{\star}, C^{\star} \subseteq \real^{d \times r}$ and a quadratic function $\kappa$ with kernel $K \subseteq \real^{3 \times 3}$.
	Assume that $\max(\norm{e_i^{\top} A^{\star}}, \norm{e_i^{\top} B^{\star}}, \norm{e_i^{\top} C^{\star}}) \le \sqrt{\alpha}$, for all $1 \le i \le d$.
	We are given a uniformly random subset of $m$ entries $\Omega \subseteq [d]^3$ from $T^{\star}$, along with their values.
	Let $C \in \cS_{3d}^+$ be a random PSD matrix with spectral norm at most $\lambda_1$ and
	\[ g(X,Y,Z) = h(X,Y,Z) + \inner{[X;Y;Z]}{C \dot [X;Y;Z]}. \]
	Let $m \gtrsim d (\log d) / \varepsilon^2$ and $R \ge \sqrt{2m + 2d}$.
	For any local minimum $X,Y,Z$ of $g$, with high probability over the randomness of $\Omega$ and $C$, by reconstructing $\hat{T}_{i, j, k} = \sum_{l=1}^R \kappa(X_{i,l}, Y_{j,l}, Z_{k,l})$, we have:
	\[ \frac 1 {d^3} \normFro{\hat{T} - T^{\star}}^2 \lesssim \alpha^2 \varepsilon. \]
\end{theorem}

Note that Theorem \ref{thm_intro} is a specal case of Theorem \ref{thm_main}.
This is because when $\norm{A}_{\infty} \le \sqrt{\alpha}$, we have that $\norm{e_i^{\top} A} \le \sqrt{r\alpha}$ for all $1 \le i \le d$.
The same holds for $B$ and $C$.
Hence Theorem \ref{thm_intro} follows by setting $\alpha = \sqrt{r\alpha}$ in Theorem \ref{thm_main}.

As another example, suppose that $A^{\star}, B^{\star}, C^{\star}$ are all sampled independently from $\cN(0, 1 / \sqrt d)$.
In this case, it is easy to verify that $\alpha = O(r (\log d) / d)$.
When $m \gtrsim d r^4 \log^3 d$, we have that the average MSE of $\hat{T}$ is at most $O(\varepsilon/ d^2)$.
Note that every entry of $T^{\star}$ is on the order of $1/d$ based on the quadratic model.
Hence $\hat{T}$ can recover $T^{\star}$ for most entries up to a relative MSE of $\varepsilon$.

The first technical complication of analyzing $h(X,Y,Z)$ is that the three factors are asymmetric.
Therefore to simplify the analysis, we first reduce the problem to a symmetric problem, by viewing the search space as $[X; Y; Z]$ instead.
We then show that all local minima of $g(X,Y,Z)$ are global minima, via an interesting connection between SDPs and ther low-rank Burer-Monteiro formulation \cite{BVB16}.
We use smoothed analysis to \todo{phrasing}.
This will ensure that any local minima incurs a small MSE on $\Omega$.
Then we bound the generalization error through the regularization added to $g(X,Y,Z)$.

\paragraph{Local optimality} Before proceeding, we introduce several notations needed in the proof.
Denote by $U^{\star} = [A^{\star}; B^{\star}; C^{\star}] \subseteq \real^{3d \times r}$ as the three factors stacked vertically.
Let $X^{\star} = U^{\star} {U^{\star}}^{\top}$.
For each triple $t = (i, j, k) \in [d]^3$, denote by $A_t \subseteq \real^{3d \times 3d}$ as a sensing matrix such that $\inner{A_t}{X^{\star}} = T^{\star}_{i, j, k}$.
Specifically, we have that $A_t$ restricted to the row and column indices $i, j+d, k+2d$ is equal to $K$ (the kernel matrix of $\kappa$), and $0$ otherwise.
\todo{draw pic?}
We can rewrite $g(X, Y, Z)$ as follows:
\begin{align}
	f(U) = \frac 1 m \sum_{t \in \Omega} \inner{A_t}{UU^{\top} - X^{\star}}^2 + \lambda_1 \normFro{U}^2
	+ \lambda_2 \sum_{i=1}^{3d} q_{\alpha}(\norm{e_i^{\top} U})
	+ \inner{C}{UU^{\top}},
\end{align}
where $U = [X;Y;Z] \subseteq \real^{3d \times R}$.

We will use the following Proposition during the proof.
\begin{proposition}[Proposition 4 in Bach et al. \cite{BMP08}]\label{prop_deficient}
		Let $g$ be a twice differentiable function convex function over $\cS_d^+$.
		If the function $h: U \rightarrow g(UU^{\top})$ defined over $U \subseteq d \times d'$ has a local minimum at a rank deficient matrix $V$, then $VV^{\top}$ is a global minimum of $g$.
\end{proposition}

Here we show that there is no bad local minima in the landscape of $g(U)$.
\begin{lemma}\label{lem_local}
	In the setting of Theorem \ref{thm_main}, we have that any local minimum $V$ of $g(U)$ is a global minimum with high probability.
\end{lemma}

\begin{proof}
	Since $V$ is a local minimum of $f(U) + \inner{C}{UU^{\top}}$, we have that $\nabla g(U) = \zeroMatrix$.
	We will show that $\rank(V) < k$, hence by Proposition \ref{prop_deficient}, $V$ is a global minimum of $g(U)$.
	Assume that $\rank(V) = k$.
	By $\nabla g(U) = \zeroMatrix$, we obtain:
	\begin{align}
		& \left(\sum_{t \in \Omega} z_t A_t
		+ \sum_{i = 1}^d w_i e_i e_i^{\top}
		+ \lambda_1 \id + C \right) U = \zeroMatrix, \\
		&\quad\quad \text{where}~ w_i = \frac{4\lambda_2 (\norm{e_i^{\top} U} -\alpha)^3} {\norm{e_i^{\top} U}} \ind{\norm{e_i^{\top} U} \ge \alpha}, \\
		&\quad\quad \text{and}~ z_t = \frac 2 m \inner{A_t}{UU^{\top} - X^{\star}}
	\end{align}
	Denote by
	\begin{align}
		& M(w, z) = \sum_{i=1}^d w_i e_i e_i^{\top} + \sum_{t \in \Omega} z_t A_t, \text{and} \\
		& \cA = \bigset{X - M(w, z) - \lambda_1 \id : X \in \cS_{3d}, XU = \zeroMatrix, w \in \real^d, z \in \real^m}.
	\end{align}
	The set $\cA$ is a manifold and we have that $C \in \cA$.
	Note that $X$ is a symmetric matrix in the null space of $U$,
	recalling that $A_t$ is a symmetric matrix, for any $t \in [d]^3$.
	Since the rank of the null space is $n - k$, the dimension of such $X$ is $\frac{3d(3d+1)} 2 - \frac{k(k+1)} 2$.
	Together with $w$ and $z$, we have that the dimension of $\cA$ is
	\[ \frac{3d(3d+1)} 2 - \frac{k(k+1)} 2 + m + d. \]
	We have assumed that $k \ge \sqrt{2m + 2d}$, implying that the dimension of $\cA$ is less than $\frac{3d(3d+1)} 2$.
	However, the probability that a random PSD matrix $C$ falls in such a set $\cA$ only happens with probability zero.
	Hence with high probability, the rank of $V$ is less than $k$.
\end{proof}

\paragraph{Rademacher complexity}
Next we bound the Rademacher complexity of quadratic tensor models.
We first introduce some notations.
For any $S \subseteq [d]^3$, denote by
\[ \cL_{S}(X) = \frac 1 {\abs{S}} \sum_{t \in S} \abs{\inner{A_t}{X - X^{\star}}}. \]
And let $\cG$ denote the set of matrices as follows.
\begin{align*}
	\cG \define \bigset{X \in \cS_{3d}^+ : \tr(X) \le 2d\alpha, X_{i, i} \le 2\alpha ~\forall~ 1 \le i \le d}.
\end{align*}
We bound the Rademacher complexity of $\cG$ in the following Lemma.
\begin{lemma}\label{lem_rade}
	In the setting of Theorem \ref{thm_main}, we have that with high probability over the randomness of $\Omega$,
	\[ \sup_{X \in \cG} \abs{\cL_{\Omega}(X) - \cL_{[d]^3}(X)} \le c \norm{K}_1 \alpha^2 \varepsilon, \]
	where $c$ is a certain fixed constant.
\end{lemma}

\begin{proof}%
	We will prove the following inequality:
	\begin{align}\label{eq_markov}
		\left( \exarg{\Omega}{\sup_{X \in \cG} \abs{\cL_{\Omega}(X) - \cL_{[d]^3}(X)}^h}
	\right)^{\frac 1 h} \le {c_1 \norm{K}_1 \alpha^2 \sqrt{\frac d m + \frac{d^{2}\log d}{m^2}}}
		\le {c_1 \norm{K}_1 \alpha^2 \varepsilon}.
	\end{align}
	Based on the above inequality, we can obtain the desired conclusion by using markov's inequality, setting $c = 2c_1$ and $h = \log d$.
	\begin{align}
		\Pr\bigbrace{\sup_{X \in \cG} \abs{\cL_{\Omega}(X) - \cL_{[d]^3}(X)}^h \ge (2c\norm{K}\alpha^2\varepsilon)^h}
		\le \frac 1 {2^h} = \frac 1 d.
	\end{align}
	Let $\Omega'$ denote a set of $m$ independent samples from $[d]^3$.
	Clearly,
	\[ \exarg{\Omega}{\cL_{\Omega}(X)} = \exarg{\Omega'}{\cL_{\Omega'}(X)}. \]
	Note that taking the power of $h$ is a convex function and the supremum over $\cG$ is also a convex operation.
	Hence by Jensen's inequality, we have:
	\begin{align}
		& \exarg{\Omega}{\sup_{X \in \cG} \abs{\frac 1 m \sum_{t \in \Omega} \inner{A_t}{X - X^{\star}}^2  - \exarg{\Omega'}{\frac 1 m \sum_{t' \in \Omega'} \inner{A_{t'}}{X - X^{\star}}^2} }^h } \\
		\le & \exarg{\Omega, \Omega'}{\sup_{X \in \cG} \abs{\frac 1 m \sum_{t \in \Omega} \inner{A_t}{X - X^{\star}}^2 - \frac 1 m \sum_{t' \in \Omega'} \inner{A_{t'}}{X - X^{\star}}^2}^h}
		\label{eq_jensen}
	\end{align}
	Let $\set{\sigma_i}_{i=1}^m$ denote $m$ i.i.d. Rademacher random variables.
	By the symmetry of $\Omega$ and $\Omega'$, Equation \eqref{eq_jensen} is equal to:
	\begin{align}
		& \exarg{\Omega, \Omega', \sigma}{\sup_{X \in \cG} \abs{\frac 1 m \sum_{l=1}^m \sigma_l \times \bigbrace{\inner{A_{t_l}}{X - X^{\star}}^2 - \inner{A_{t'_l}}{X - X^{\star}}^2} }^h} \\
		& \le	2^h \times \exarg{\Omega, \sigma}{\sup_{X \in \cG} \abs{\frac 1 m \sum_{l=1}^m \sigma_l \inner{A_{t_l}}{X - X^{\star}}^2}^h} \\
		&\le 4^h \bigbrace{ \exarg{\Omega, \sigma}{\sup_{X \in \cG} \abs{\frac 1 m \sum_{l=1}^m \sigma_l \inner{A_{t_l}}{X} (\inner{A_{t_l}}{X - 2X^{\star}})}^h}
		+ \exarg{\Omega, \sigma}{\abs{\frac 1 m \sum_{l=1}^m \sigma_l \inner{A_{t_l}}{X^{\star}}^2}^h}} \label{eq_sum}
	\end{align}
	by the symmetry between $\Omega$ and $\Omega'$ and Holder's inequality.
	We will focus on the first part of the above Equation, since the second part can be bounded similarly, noting that $X^{\star} \in \cG$.

	To bound the first part inEquation \eqref{eq_sum}, we use the Ledoux-Talagrand contraction inequality (Theorem 4.12 in \cite{LT13}).
	Consider the function $\inner{A_t}{X - X^{\star}}$ within the set $X \in \cG$.


	For any $X \in \cG$, we clearly have that for any $t \in \Omega$, $\abs{\inner{A_t}{X}} \le \norm{X}_{\infty} \norm{K}_{1} \le 2\alpha \norm{K}_1$.
	Also, because we assume that $\norm{X^{\star}}_{\infty} \le \alpha$,
	$\abs{\inner{A_t}{X^{\star}}} \le \alpha \norm{K}_{1}$.
	Hence for any $t \in [d]^3$, we have $\inner{A_t}{X - X^{\star}} \lesssim \alpha\norm{K}_1$.

	Equation can be bounded by $O({\alpha \norm{K}_1}/ {m})^h$ times the following.
	\begin{align}
		& \exarg{\Omega, \sigma}{\sup_{X \in \cG} \abs{\sum_{l=1}^m \sigma_l \inner{A_l}{X - X^{\star}}}^h} \\
		\le & \exarg{\Omega, \sigma}{\sup_{X \in \cG} \bigbrace{\tr(X + X^{\star})^h \bignorm{\sum_{l=1}^m \sigma_l A_l}^h}} \\
		\le & \bigo{d\alpha}^h \exarg{\Omega, \sigma}{\bignorm{\sum_{l=1}^m \sigma_l A_l}^h} \\
		\le & \bigo{d \alpha \sqrt{\frac m d}}^h \tag{Holder's inequality \todo{add detail}}
	\end{align}
	Equation \eqref{eq_markov} follows from the above, multiplying back $O(\alpha \norm{K}_1 / m)^d$ with the above.
	Hence the proof is complete.
\end{proof}

Lastly, we finish the proof of Theorem \ref{thm_main}.

\begin{proof}[Proof of Theorem \ref{thm_main}]
	By Lemma \ref{lem_local}, we have that $V$ is a global minimum of $g(U)$.
	In particular, this implies that
	\[ g(V) \le g(U^{\star}) \le (\lambda_1 + \norm{C}) \normFro{U^{\star}}^2 \le 2\lambda_1 \normFro{U^{\star}}, \]
	since $\normFro{C} \le \lambda_1$.
	In particular, this implies that the training error $\cL_{\Omega}(VV^{\top}) \le 2\lambda \normFro{U^{\star}}^2 \lesssim \norm{K}_1 \alpha^2 \varepsilon$ by the setting of $\lambda_1$.

	We also obtain that $\norm{e_i^{\top} V} \le \sqrt 2 \alpha$ by the setting of $\lambda_2$.
	Hence we conclude that the $(i,i)$-th entry of $VV^{\top}$ is at most $2\alpha$ and its trace is at most $2d\alpha$.
	This implies that $VV^{\top} \in \cG$.
	Hence by Lemma \ref{lem_rade}, the generalization error is also bounded by $\bigo{\norm{K}_1 \alpha^2 \varepsilon}$.
	The proof is complete.
\end{proof}


\paragraph{Discussion.} Room for improvement over k?








==> pairwise_seri.tex <==
\section{Recovery Guarantee for Quadratic Tensor Models}
\label{sec_main}

In this section, we consider the recovery of quadratic tensor models given only partial observations.
Recall that we observe $m$ uniformly random entries from the unknown tensor $T$.
Let $\Omega \in [d]^3$ denote the indices of the set of observed entries.
Given the set of observations $\Omega$, our goal is to recover $T$.
We first review the definition of local optimality conditions.

\begin{definition}
	(Local minimum) Suppose that $U$ is a local minimum of $f(U)$, then we have that
	$\nabla f(U) = \zeroMatrix$ and $\nabla^2 f(U) \gematrix \zeroMatrix$.
\end{definition}

We focus on the following non-convex formulation
over the set of $X,Y,Z \subseteq \real^{d \times R}$.
\begin{align}
	\min_{X,Y,Z \subseteq \real^{d \times R}} h(X,Y,Z) = & \frac 1 m \sum_{(i, j, k) \in \Omega} \bigbrace{\sum_{l=1}^R \kappa(X_{i,l}, Y_{j,l}, Z_{k,l}) - T_{i, j, k}}^2 \\
	+ & \lambda_1 (\normFro{X}^{2} + \normFro{Y}^2 + \normFro{Z}^2) \\
	+ & \lambda_2 \sum_{i=1}^d q_{\alpha}(\norm{e_i^{\top} U}),
\end{align}
where $q_{\alpha}(x) = (\abs{x} - \sqrt{\alpha})^4 \ind{x \ge \sqrt{\alpha}}$,
$\lambda_1 = \bigo{\frac{\norm{K} \mu} {d^2} \sqrt{\frac d m}}$ and $\lambda_2 = \frac{d^2 r} {\mu^4} \lambda_1$ (the reason for the setting will be clear later).
Here $q_{\alpha}(x)$ acts as a regularizer which penalizes the rows of $A,B,C$ whose norms are larger than $\sqrt{\alpha}$.
And the $l_2$ regularier is to ensure good generalization performance.
It is not hard to verify that $q_{\alpha}(x)$ is twice differentiable.
And it follows that $f$ is a twice differentiable function.
Our main result is described below.

\begin{theorem}\label{thm_main}
	Let $T^{\star} \subseteq \real^{d \times d \times d}$ be a quadratic tensor defined by factors $A^{\star}, B^{\star}, C^{\star} \subseteq \real^{d \times r}$ and a quadratic function $\kappa$ with kernel $K \subseteq \real^{3 \times 3}$.
	Assume that $\max(\norm{e_i^{\top} A^{\star}}, \norm{e_i^{\top} B^{\star}}, \norm{e_i^{\top} C^{\star}}) \le \sqrt{\alpha}$, for all $1 \le i \le d$.
	We are given a uniformly random subset of $m$ entries $\Omega \subseteq [d]^3$ from $T^{\star}$, along with their values.
	Let $C \in \cS_{3d}^+$ be a random PSD matrix with spectral norm at most $\lambda_1$ and
	\[ g(X,Y,Z) = h(X,Y,Z) + \inner{[X;Y;Z]}{C \dot [X;Y;Z]}. \]
	Let $m \gtrsim d (\log d) / \varepsilon^2$ and $R \ge \sqrt{2m + 2d}$.
	For any local minimum $X,Y,Z$ of $g$, with high probability over the randomness of $\Omega$ and $C$, by reconstructing $\hat{T}_{i, j, k} = \sum_{l=1}^R \kappa(X_{i,l}, Y_{j,l}, Z_{k,l})$, we have:
	\[ \frac 1 {d^3} \normFro{\hat{T} - T^{\star}}^2 \lesssim \alpha^2 \varepsilon. \]
\end{theorem}

Note that Theorem \ref{thm_intro} is a specal case of Theorem \ref{thm_main}.
This is because when $\norm{A}_{\infty} \le \sqrt{\alpha}$, we have that $\norm{e_i^{\top} A} \le \sqrt{r\alpha}$ for all $1 \le i \le d$.
The same holds for $B$ and $C$.
Hence Theorem \ref{thm_intro} follows by setting $\alpha = \sqrt{r\alpha}$ in Theorem \ref{thm_main}.

As another example, suppose that $A^{\star}, B^{\star}, C^{\star}$ are all sampled independently from $\cN(0, 1 / \sqrt d)$.
In this case, it is easy to verify that $\alpha = O(r (\log d) / d)$.
When $m \gtrsim d r^4 \log^3 d$, we have that the average MSE of $\hat{T}$ is at most $O(\varepsilon/ d^2)$.
Note that every entry of $T^{\star}$ is on the order of $1/d$ based on the quadratic model.
Hence $\hat{T}$ can recover $T^{\star}$ for most entries up to a relative MSE of $\varepsilon$.

The first technical complication of analyzing $h(X,Y,Z)$ is that the three factors are asymmetric.
Therefore to simplify the analysis, we first reduce the problem to a symmetric problem, by viewing the search space as $[X; Y; Z]$ instead.
We then show that all local minima of $g(X,Y,Z)$ are global minima, via an interesting connection between SDPs and ther low-rank Burer-Monteiro formulation \cite{BVB16}.
We use smoothed analysis to \todo{phrasing}.
This will ensure that any local minima incurs a small MSE on $\Omega$.
Then we bound the generalization error through the regularization added to $g(X,Y,Z)$.

\paragraph{Local optimality} Before proceeding, we introduce several notations needed in the proof.
Denote by $U^{\star} = [A^{\star}; B^{\star}; C^{\star}] \subseteq \real^{3d \times r}$ as the three factors stacked vertically.
Let $X^{\star} = U^{\star} {U^{\star}}^{\top}$.
For each triple $t = (i, j, k) \in [d]^3$, denote by $A_t \subseteq \real^{3d \times 3d}$ as a sensing matrix such that $\inner{A_t}{X^{\star}} = T^{\star}_{i, j, k}$.
Specifically, we have that $A_t$ restricted to the row and column indices $i, j+d, k+2d$ is equal to $K$ (the kernel matrix of $\kappa$), and $0$ otherwise.
\todo{draw pic?}
We can rewrite $g(X, Y, Z)$ as follows:
\begin{align}
	f(U) = \frac 1 m \sum_{t \in \Omega} \inner{A_t}{UU^{\top} - X^{\star}}^2 + \lambda_1 \normFro{U}^2
	+ \lambda_2 \sum_{i=1}^{3d} q_{\alpha}(\norm{e_i^{\top} U})
	+ \inner{C}{UU^{\top}},
\end{align}
where $U = [X;Y;Z] \subseteq \real^{3d \times R}$.

We will use the following Proposition during the proof.
\begin{proposition}[Proposition 4 in Bach et al. \cite{BMP08}]\label{prop_deficient}
		Let $g$ be a twice differentiable function convex function over $\cS_d^+$.
		If the function $h: U \rightarrow g(UU^{\top})$ defined over $U \subseteq d \times d'$ has a local minimum at a rank deficient matrix $V$, then $VV^{\top}$ is a global minimum of $g$.
\end{proposition}

Here we show that there is no bad local minima in the landscape of $g(U)$.
\begin{lemma}\label{lem_local}
	In the setting of Theorem \ref{thm_main}, we have that any local minimum $V$ of $g(U)$ is a global minimum with high probability.
\end{lemma}

\begin{proof}
	Since $V$ is a local minimum of $f(U) + \inner{C}{UU^{\top}}$, we have that $\nabla g(U) = \zeroMatrix$.
	We will show that $\rank(V) < k$, hence by Proposition \ref{prop_deficient}, $V$ is a global minimum of $g(U)$.
	Assume that $\rank(V) = k$.
	By $\nabla g(U) = \zeroMatrix$, we obtain:
	\begin{align}
		& \left(\sum_{t \in \Omega} z_t A_t
		+ \sum_{i = 1}^d w_i e_i e_i^{\top}
		+ \lambda_1 \id + C \right) U = \zeroMatrix, \\
		&\quad\quad \text{where}~ w_i = \frac{4\lambda_2 (\norm{e_i^{\top} U} -\alpha)^3} {\norm{e_i^{\top} U}} \ind{\norm{e_i^{\top} U} \ge \alpha}, \\
		&\quad\quad \text{and}~ z_t = \frac 2 m \inner{A_t}{UU^{\top} - X^{\star}}
	\end{align}
	Denote by
	\begin{align}
		& M(w, z) = \sum_{i=1}^d w_i e_i e_i^{\top} + \sum_{t \in \Omega} z_t A_t, \text{and} \\
		& \cA = \bigset{X - M(w, z) - \lambda_1 \id : X \in \cS_{3d}, XU = \zeroMatrix, w \in \real^d, z \in \real^m}.
	\end{align}
	The set $\cA$ is a manifold and we have that $C \in \cA$.
	Note that $X$ is a symmetric matrix in the null space of $U$,
	recalling that $A_t$ is a symmetric matrix, for any $t \in [d]^3$.
	Since the rank of the null space is $n - k$, the dimension of such $X$ is $\frac{3d(3d+1)} 2 - \frac{k(k+1)} 2$.
	Together with $w$ and $z$, we have that the dimension of $\cA$ is
	\[ \frac{3d(3d+1)} 2 - \frac{k(k+1)} 2 + m + d. \]
	We have assumed that $k \ge \sqrt{2m + 2d}$, implying that the dimension of $\cA$ is less than $\frac{3d(3d+1)} 2$.
	However, the probability that a random PSD matrix $C$ falls in such a set $\cA$ only happens with probability zero.
	Hence with high probability, the rank of $V$ is less than $k$.
\end{proof}

\paragraph{Rademacher complexity}
Next we bound the Rademacher complexity of quadratic tensor models.
We first introduce some notations.
For any $S \subseteq [d]^3$, denote by
\[ \cL_{S}(X) = \frac 1 {\abs{S}} \sum_{t \in S} \abs{\inner{A_t}{X - X^{\star}}}. \]
And let $\cG$ denote the set of matrices as follows.
\begin{align*}
	\cG \define \bigset{X \in \cS_{3d}^+ : \tr(X) \le 2d\alpha, X_{i, i} \le 2\alpha ~\forall~ 1 \le i \le d}.
\end{align*}
We bound the Rademacher complexity of $\cG$ in the following Lemma.
\begin{lemma}\label{lem_rade}
	In the setting of Theorem \ref{thm_main}, we have that with high probability over the randomness of $\Omega$,
	\[ \sup_{X \in \cG} \abs{\cL_{\Omega}(X) - \cL_{[d]^3}(X)} \le c \norm{K}_1 \alpha^2 \varepsilon, \]
	where $c$ is a certain fixed constant.
\end{lemma}

\begin{proof}[Proof of Lemma \ref{lem_rade}]
	We will prove the following inequality:
	\begin{align}\label{eq_markov}
		\left( \exarg{\Omega}{\sup_{X \in \cG} \abs{\cL_{\Omega}(X) - \cL_{[d]^3}(X)}^h}
	\right)^{\frac 1 h} \le {c_1 \norm{K}_1 \alpha^2 \sqrt{\frac d m + \frac{d^{2}\log d}{m^2}}}
		\le {c_1 \norm{K}_1 \alpha^2 \varepsilon}.
	\end{align}
	Based on the above inequality, we can obtain the desired conclusion by using markov's inequality, setting $c = 2c_1$ and $h = \log d$.
	\begin{align}
		\Pr\bigbrace{\sup_{X \in \cG} \abs{\cL_{\Omega}(X) - \cL_{[d]^3}(X)}^h \ge (2c\norm{K}\alpha^2\varepsilon)^h}
		\le \frac 1 {2^h} = \frac 1 d.
	\end{align}
	Let $\Omega'$ denote a set of $m$ independent samples from $[d]^3$.
	Clearly,
	\[ \exarg{\Omega}{\cL_{\Omega}(X)} = \exarg{\Omega'}{\cL_{\Omega'}(X)}. \]
	Note that taking the power of $h$ is a convex function and the supremum over $\cG$ is also a convex operation.
	Hence by Jensen's inequality, we have:
	\begin{align}
		& \exarg{\Omega}{\sup_{X \in \cG} \abs{\frac 1 m \sum_{t \in \Omega} \inner{A_t}{X - X^{\star}}^2  - \exarg{\Omega'}{\frac 1 m \sum_{t' \in \Omega'} \inner{A_{t'}}{X - X^{\star}}^2} }^h } \\
		\le & \exarg{\Omega, \Omega'}{\sup_{X \in \cG} \abs{\frac 1 m \sum_{t \in \Omega} \inner{A_t}{X - X^{\star}}^2 - \frac 1 m \sum_{t' \in \Omega'} \inner{A_{t'}}{X - X^{\star}}^2}^h}
		\label{eq_jensen}
	\end{align}
	Let $\set{\sigma_i}_{i=1}^m$ denote $m$ i.i.d. Rademacher random variables.
	By the symmetry of $\Omega$ and $\Omega'$, Equation \eqref{eq_jensen} is equal to:
	\begin{align}
		& \exarg{\Omega, \Omega', \sigma}{\sup_{X \in \cG} \abs{\frac 1 m \sum_{l=1}^m \sigma_l \times \bigbrace{\inner{A_{t_l}}{X - X^{\star}}^2 - \inner{A_{t'_l}}{X - X^{\star}}^2} }^h} \\
		& \le	2^h \times \exarg{\Omega, \sigma}{\sup_{X \in \cG} \abs{\frac 1 m \sum_{l=1}^m \sigma_l \inner{A_{t_l}}{X - X^{\star}}^2}^h} \\
		&\le 4^h \bigbrace{ \exarg{\Omega, \sigma}{\sup_{X \in \cG} \abs{\frac 1 m \sum_{l=1}^m \sigma_l \inner{A_{t_l}}{X} (\inner{A_{t_l}}{X - 2X^{\star}})}^h}
		+ \exarg{\Omega, \sigma}{\abs{\frac 1 m \sum_{l=1}^m \sigma_l \inner{A_{t_l}}{X^{\star}}^2}^h}} \label{eq_sum}
	\end{align}
	by the symmetry between $\Omega$ and $\Omega'$ and Holder's inequality.
	We will focus on the first part of the above Equation, since the second part can be bounded similarly, noting that $X^{\star} \in \cG$.

	To bound the first part inEquation \eqref{eq_sum}, we use the Ledoux-Talagrand contraction inequality (Theorem 4.12 in \cite{LT13}).
	Consider the function $\inner{A_t}{X - X^{\star}}$ within the set $X \in \cG$.


	For any $X \in \cG$, we clearly have that for any $t \in \Omega$, $\abs{\inner{A_t}{X}} \le \norm{X}_{\infty} \norm{K}_{1} \le 2\alpha \norm{K}_1$.
	Also, because we assume that $\norm{X^{\star}}_{\infty} \le \alpha$,
	$\abs{\inner{A_t}{X^{\star}}} \le \alpha \norm{K}_{1}$.
	Hence for any $t \in [d]^3$, we have $\inner{A_t}{X - X^{\star}} \lesssim \alpha\norm{K}_1$.

	Equation can be bounded by $O({\alpha \norm{K}_1}/ {m})^h$ times the following.
	\begin{align}
		& \exarg{\Omega, \sigma}{\sup_{X \in \cG} \abs{\sum_{l=1}^m \sigma_l \inner{A_l}{X - X^{\star}}}^h} \\
		\le & \exarg{\Omega, \sigma}{\sup_{X \in \cG} \bigbrace{\tr(X + X^{\star})^h \bignorm{\sum_{l=1}^m \sigma_l A_l}^h}} \\
		\le & \bigo{d\alpha}^h \exarg{\Omega, \sigma}{\bignorm{\sum_{l=1}^m \sigma_l A_l}^h} \\
		\le & \bigo{d \alpha \sqrt{\frac m d}}^h \tag{Holder's inequality \todo{add detail}}
	\end{align}
	Equation \eqref{eq_markov} follows from the above, multiplying back $O(\alpha \norm{K}_1 / m)^d$ with the above.
	Hence the proof is complete.
\end{proof}

Lastly, we finish the proof of Theorem \ref{thm_main}.

\begin{proof}[Proof of Theorem \ref{thm_main}]
	By Lemma \ref{lem_local}, we have that $V$ is a global minimum of $g(U)$.
	In particular, this implies that
	\[ g(V) \le g(U^{\star}) \le (\lambda_1 + \norm{C}) \normFro{U^{\star}}^2 \le 2\lambda_1 \normFro{U^{\star}}, \]
	since $\normFro{C} \le \lambda_1$.
	In particular, this implies that the training error $\cL_{\Omega}(VV^{\top}) \le 2\lambda \normFro{U^{\star}}^2 \lesssim \norm{K}_1 \alpha^2 \varepsilon$ by the setting of $\lambda_1$.

	We also obtain that $\norm{e_i^{\top} V} \le \sqrt 2 \alpha$ by the setting of $\lambda_2$.
	Hence we conclude that the $(i,i)$-th entry of $VV^{\top}$ is at most $2\alpha$ and its trace is at most $2d\alpha$.
	This implies that $VV^{\top} \in \cG$.
	Hence by Lemma \ref{lem_rade}, the generalization error is also bounded by $\bigo{\norm{K}_1 \alpha^2 \varepsilon}$.
	The proof is complete.
\end{proof}


\paragraph{Discussion.} Room for improvement over k?







